What makes nonholonomic integrators work?

A nonholonomic system is a mechanical system with velocity constraints not originating from position constraints; rolling without slipping is the typical example. A nonholonomic integrator is a numerical method specifically designed for nonholonomic systems. It has been observed numerically that many nonholonomic integrators exhibit excellent long-time behaviour when applied to various test problems. The excellent performance is often attributed to some underlying discrete version of the Lagrange--d'Alembert principle. Instead, in this paper, we give evidence that reversibility is behind the observed behaviour. Indeed, we show that many standard nonholonomic test problems have the structure of being foliated over reversible integrable systems. As most nonholonomic integrators preserve the foliation and the reversible structure, near conservation of the first integrals is a consequence of reversible KAM theory. Therefore, to fully evaluate nonholonomic integrators one has to consider also non-reversible nonholonomic systems. To this end we construct perturbed test problems that are integrable but no longer reversible (with respect to the standard reversibility map). Applying various nonholonomic integrators from the literature to these problems we observe that no method performs well on all problems. This further indicates that reversibility is the main mechanism behind near conservation of first integrals for nonholonomic integrators. A list of relevant open problems is given.

==> chaplygin.tex <==

The Lagrangian and the constraints are given by:
\begin{align}
	\Lag = \frac{1}{2}\paren[\big]{{\vx}^2 + {\vy}^2 + {\dot{\theta}^2}} \\
-\sin(\theta)\vx + \cos(\theta) \vy - \dot{\theta} = 0
\end{align}
% It does not fit in the framework above because of the presence of $\dot{\theta}$ in the constraint.

\newcommand*\etheta{\ee^{\ii\theta}}

For convenience, we denote $z \coloneqq x + \ii y$, and $\omega \coloneqq \dot{\theta}$, $v \coloneqq z'$.
The Lagrange--d'Alembert equations become
\begin{align}
	z' &= v\\
	\theta' &= \omega\\
	v' &= \ii \etheta \lambda\\
	\omega' &= - \lambda
\end{align}
The nonholonomic constraint is
\begin{align}
\scalprod{\ii \etheta}{ v} = \omega
,
\end{align}
where $\scalprod{\cdot}{\cdot}$ denotes the scalar product in $\RR^2 \equiv \CC$.

Define the variable $p \coloneqq \scalprod{\etheta}{v}$.
By differentiating, we obtain
\begin{align}
p' &= \scalprod{\theta' \ii \etheta}{v} + \scalprod{\etheta}{v'}\\
&= \omega \scalprod{\ii \etheta}{v} + \scalprod{\etheta}{\ii\etheta}\lambda \\
&=  \omega^2
\end{align}

Using the constraint, we notice that
\begin{align}
	\abs{v}^2 = {p}^2 + {\scalprod{v}{\ii\etheta}}^2 = p^2 + \omega^2
	,
\end{align}
so the energy $H = \frac{1}{2}\abs{v}^2 + \frac{1}{2}\abs{\omega}$ becomes
\begin{align}
H = \frac{1}{2}p^2 + \omega^2
.
\end{align}


By differentiating,  we have
\begin{align}
H' = p p' + 2 \omega' \omega = p\omega^2 + 2 \omega' \omega = 0
,
\end{align}
from which we deduce that $\omega' = -\frac{1}{2}p \omega$.

So, the reduced system is
\begin{align}
	\label{eq:chaplyginaa}
p' &= \omega^2\\
\omega' &= -\frac{1}{2}p\omega
          .
\end{align}

As \(\dd H = p\dd p + 2 \omega \dd \omega\),
if $\Pi = -\frac{1}{2} \omega \frac{\partial}{\partial p} \wedge \frac{\partial}{\partial \omega}$, we see that $\pairing{\Pi}{\dd H} = -\frac{1}{2}\omega p \frac{\partial}{\partial \omega} + \omega^2 \frac{\partial}{\partial p}$.
We thus see that the reduced system is Poisson with respect to the Poisson structure $\Pi$.
Note that $\Pi$ is the Lie--Poisson structure associated to the Lie algebra of the one dimensional affine group.

We also note that if $R(p,\omega) = (-p, \omega)$, then the vector field is such that $RX(R(p,\omega)) = -\omega^2 \frac{\partial}{\partial p} + \frac{1}{2}p\omega\frac{\partial}{\partial \omega} = - X$, and $H$ is $R$-invariant, so the system is $R$-integrable.

As
\(
H = \frac{1}{2}p^2 + \omega^2 
\)
is a first integral of the two-dimensional system~\eqref{eq:chaplyginaa}, that system is integrable.

A complete system of equations is
\begin{align}
 z' &= v \\ 
\theta' &= \omega \\
p' &= \omega^2\\
\omega' &= -\frac{1}{2}p \omega
\end{align}
The Chaplygin sleigh is thus of a type similar to the systems studied in \autoref{sec:nonholexamples}: the fibres have dimension $3$, the underlying integrable system has one invariant, $H$, and one angle variable.
The projection to the reduced system is $\pi\colon (z,\theta,p,\omega) \mapsto (p, \omega)$.

==> discrete_integral.tex <==


The method is
\begin{align}
  \xx_1 &= \xx_0 + h \dot{\xx}_1 \\
\dot{\xx}_1 &= \dot{\xx}_0 + h(-\nabla V(\xx_0)) + A(\zz_0)^T\lambda \\
A(\zz_0)(\dot{\xx}_0 + \dot{\xx}_1) &= 0
\end{align}


By multiplying by $\dot{\xx}_0 + \dot{\xx}_1$ we obtain
\begin{equation}
  \norm{\dot{\xx}_1}^2 - \norm{\dot{\xx}_0}^2 = -h\paren[\big]{(\dot{\xx}_0+\dot{\xx}_1),\nabla V(\xx_0)}
  .
\end{equation}
% We now define $\vv_i$ by $\dot{\xx_i} = \vv_i \kker(\zz_i)$, so in particular, $\vv_i = \norm{\dot{\xx_i}}$.
We define $\vv_i = \norm{\dot{\xx_i}}$.
Using also $h\dot{\xx_i} = \xx_i - \xx_{i-1}$ now gives
\begin{equation}
  {\vv_1}^2 - {\vv_0}^2 = - \paren[\big]{\xx_1 - \xx_{-1}, \nabla V(\xx_0)}
  .
\end{equation}

If $V$ is quadratic, this yields
\begin{equation}
  \vv_1^2 - \vv_0^2 = - \xx_1 \xx_0 + \xx_{-1}\xx_0
\end{equation}
This gives conservation of
\begin{equation}
  \vv_1^2 + \xx_1\xx_0
\end{equation}
We rewrite this into
\begin{equation}
  \vv_1^2 + \frac{1}{4}\paren[\big]{\norm{\xx_1 + \xx_0}^2 - \norm{\xx_1 - \xx_0}^2}
\end{equation}
which gives conservation of
\begin{equation}
  \mathcal{E} = \paren[\Big]{1 - \frac{h^2}{4}}\vv_1^2 + \norm[\Big]{\frac{\xx_1 + \xx_0}{2}}^2
\end{equation}
We rewrite it as
\begin{equation}
  \mathcal{E} = \paren[\Big]{1 - \frac{h^2}{4}}\vv_1^2 + \norm[\Big]{\xx_1 - h \dot\xx_1/2}^2
  .
\end{equation}
In particular, this gives a bound on $\vv_1$.
Observe that
\begin{equation}
 \norm{\xx_1} - h \abs{\vv_1}/2 \leq \norm{\xx_1 - h \dot{\xx_1}/2} 
% \leq \norm{\xx_1} + h \abs{\vv_1}/2
\end{equation}
As we have a bound $B$ on $\vv_1$, and a bound on $ \norm[\big]{\xx_1 - h \dot\xx_1/2}^2$, we get a bound $C$ on $\norm{\xx_1}$, so the energy is bounded.
% On the other hand, we also have $\mathcal{E} \leq \vv_1^2 + \norm{\xx_1}^2 + hBC h B^2/4$, so the energy is also bounded below.

% \itodo[OV]{From this formulation, it should be possible to give explicit bounds on the quantity $\vv_i^2 + \norm{\xx_i}^2$, depending on $\mathcal{E}$ and $h$}

==> table.tex <==

\newcommand*\mmidrule{\arrayrulecolor{gray!50}\midrule\arrayrulecolor{black}}

\afterpage{
	\clearpage
\begin{landscape}
  \centering
  \begin{tabular}[t]{p{3cm}l|cc|ccccc|ccc|c}
    \toprule
		\rowcolor{Linen}
    System 
& $\S$
& $\xx\in$
& $\zz\in$
& Group
&$\smallV(\zz)$ 
    & $\consmat(\zz)$
& $\hstiff$ 
& $\FF$
& $F$ & $I$ & $\theta$
              & $\rho$
\\ \midrule
CVT
& \autoref{sec:cvt}
  & $\RR^2$
& $\RR$
& $\SO(3)$ 
& $\zz^2/2$ 
&$\begin{bmatrix}
		1 & \zz
	\end{bmatrix}$ 
&$\begin{bmatrix}
		1 & 0\\0 &1
	\end{bmatrix}$
& $0$
    & $0$ & $3$ & $2$
    & $(\yy, -\vv)$
    \\
Pendulum CVT
    &
      & $\RR^2$
        & $\TT$
& $\SO(3)$ & $\cos(\zz) - \varepsilon\sin(2\zz)/2$ 
&$\begin{bmatrix}
		1 & \sin(\zz)
	\end{bmatrix}$ 
&$\begin{bmatrix}
		1 & 0\\0 &1
	\end{bmatrix}$
& $0$
    & $0$ & $3$ & $2$
    \\
% Nonholonomic 
Particle 
& 
  & $\RR^2$
& $\RR$
& $\SO(2)$ & $\zz^2/2$ 
&$\begin{bmatrix}
		1 & \zz
	\end{bmatrix}$ 
& $\begin{bmatrix}
		 0&1
	\end{bmatrix}$ 
& $0$
& $1$ & $2$ & $2$ 
\\ \mmidrule
Knife Edge 
    & \autoref{sec:knifeedge}
      & $\RR^2$
        & $\TT$
& $\RR$ 
& $0$
& $\begin{bmatrix}
		-\sin(\zz) & \cos(\zz)
	\end{bmatrix}$
& $0$
& $\begin{pmatrix}0,-1\end{pmatrix}$
& $2$ & $2$ & $1$
              & $\vv$
 \\ \mmidrule
Mobile Robot 
& \autoref{sec:verticalrollingdisk}
  & 
    &
& 
& $\sin(\zz)$ 
& 
&
&
    & $2$ & $2$ & $1$
                  & $\vv$
    \\
Rolling Disk 
& 
& \multirow{-2}*{$\RR^2\times\TT$}
& \multirow{-2}*{$\TT$}
 &  \multirow{-2}*{$\one$}
& $0$ 
& \multirow{-2}*{$\begin{bmatrix}
		1&0 &\cos(\zz)\\
		0&1&\sin(\zz)
	\end{bmatrix}$}
& \multirow{-2}*{0}
& \multirow{-2}*{0}
& $2$ & $2$ & $1$ \\
    \bottomrule
  \end{tabular}
  \captionof{table}{
Summary of the nonholonomically coupled systems presented in \autoref{sec:nonholcoupled}.
$F$ is the dimension of the kernel of $\hstiff$, and hence the dimension of the fibres of the map $\pi$ defined by equation \eqref{eq:projection}.
$I$ is the number of first integrals.
$\theta$ is the number of angle variables.
$\rho$ is the map used to define the reversibility map in \eqref{eq:Rdef}.
}
  \label{tab:summary}
\end{landscape}
}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "elbar2"
%%% End:
